Energy Optimal Point-to-Point Motion Profile Optimization

Position-controlled systems driving repetitive tasks are of significant importance in industrial machinery. The electric actuators used in these systems are responsible for a large part of the global energy consumption, indicating that major savings can be made in this field. In this context, motion profile optimization is a very cost-effective solution as it allows for more energy-efficient machines without additional hardware investments or adaptions. In particular, mono-actuated mechanisms with position-dependent system properties have received considerable attention in literature. However, the current state-of-the-art methods often use unbounded design parameters to describe the motion profile. This both increases the computational complexity and hampers the search for a global optimum. In this paper, Chebyshev polynomials are used to describe the motion profile. Moreover, the exact bounds on the Chebyshev design parameters are derived. This both seriously reduces the computational complexity and limits the design space, allowing the application of a global optimizer such as the genetic algorithm. Experiments validate the added value of the chosen approach. In this study, it is found that the energy consumption can be reduced by 62.9% compared to a standard reference motion profile.

==> Sections/04_Optimization_old.tex <==
\section{Optimization Approach}
\subsection{Motion Profile Definition \& Rescaling}
In this paper, a Chebyshev polynomial $\sum_{i=0}^{n} p_iT_i(x)$ is used to define the position profile $\theta(t)$, where $t \in [t_A,t_B]$, in between the start-$\theta(t_A) = \theta_A$ and endpoint $\theta(t_B) = \theta_B$ of the motion task. The sequence of orthogonal Chebyshev polynomials $T_n(x) = T_n(\cos(\vartheta))$, defined on the interval $x \in [-1,1]$, is obtained from the recurrence relation: 

\begin{equation} \label{eq:def_cheb}
\begin{aligned}
T_0(x) &= 1, \quad T_1(x) = x, \\
T_{k+1}(x) &= 2xT_k(x)-T_{k-1}(x),
\end{aligned}
\end{equation}

This gives exactly the same results as from the trigonometric definition:

\begin{equation} \label{eq:def_cheb_tri}
T_k(\cos(\vartheta)) = \cos(k\vartheta).
\end{equation}

%However, employing the Chebyshev polynomial as such results in infeasible solutions since the motion time interval $[t_A,t_B]$, might be outside of the valid domain of $T_n(x)$, $x \in [-1,1]$. 
To use $T_n(x)$ as a representation for the position profile, a linear transformation from $t$ into the range $[-1,1]$ of $x$ is required \cite{Thompson2013}:

\begin{equation} \label{eq:rescale_tx}
\begin{aligned}
t&=\frac{1}{2}(t_B-t_A)x+\frac{1}{2}(t_B+t_A) =a x+ b,
\end{aligned}
\end{equation}

where scale factors $a$ and $b$ are defined for the purpose of the following paragraphs. In addition, the position $\theta$ is also rescaled to the interval $[-1,1]$, which makes it possible to obtain strict bounds on the design space in \eqref{boundsDS}. Thus, the rescaled motion profile description $\phi(x)$ of degree $n$ with optimizable coefficients $\mathbf{p} = [p_0, p_1, \ldots ,p_n]^T$ is obtained.

\begin{equation} \label{eq:position_function_cheb}
\phi(x)=\sum_{i=0}^{n} p_iT_i(x), \quad x\in [-1,1].
\end{equation}

The output of the motion simulations in the previous section deliver $n_s$ samples of inertia $\mathbf{J}= [J_1, \ldots  ,J_{n_s}]^T$, load torque $\mathbf{T}_l= [T_{l,1}, \ldots  ,T_{l,n_s}]^T$ and corresponding angle query points $\boldsymbol{\uptheta} = [\theta_1, \ldots  ,\theta_{n_s}]^T$. Due to the position rescaling of the motion profile $\phi(x)$, the angle query points $\boldsymbol{\uptheta}$ of every system property vector $\mathbf{Y}$ have to be rescaled accordingly:

\begin{equation} \label{eq:rescale_prop}
\begin{aligned}
    \boldsymbol{\upphi} &= \frac{2}{(\theta_B -\theta_A)} \, \boldsymbol{\uptheta} - \frac{(\theta_B +\theta_A)}{(\theta_B -\theta_A)} = c \, \boldsymbol{\uptheta} + d.
    \end{aligned}
\end{equation}

Moreover, as the property description $Y(\phi)$ is now defined on the rescaled interval $\phi \in [-1,1]$, the following relationship holds with regard to the derivative properties:

\begin{equation} \label{eq:rescale_pder}
\frac{\mathrm{d}J(\phi)}{\mathrm{d}\phi} = \frac{1}{2}(\theta_B-\theta_A) \frac{\mathrm{d}J(\theta)}{\mathrm{d}\theta} =  e \,  \frac{\mathrm{d}J(\theta)}{\mathrm{d}\theta}.
\end{equation}

When using the rescaled position profile $\phi(x)$, it is important to rescale the torque equation \eqref{eq:torque_equation} as well. Otherwise, the resulting values of the torque profile $T(x)$ are distorted which results in different objective values (i.e. $T_{rms}$) and solutions. To preserve the motor torque's absolute values, the following rescaled torque equation is used:

\begin{equation} \label{eq:torque_equation_rescaled}
T_m(x) = T_l(\phi) + \frac{1}{2}\frac{\mathrm{d}J(\phi)}{\mathrm{d}\phi}\frac{1}{e}\left(\frac{\dot{\phi}}{a.c}\right)^2 + J(\theta)\frac{\ddot{\phi}}{a^2.c} + \mu_k\frac{\dot{\phi}}{a}.
\end{equation}

An overview of the position and torque rescalings is presented in Fig. \ref{fig:rescaling}. The new system equation \eqref{eq:torque_equation_rescaled} ensures the system dynamics are equally scaled and the minima are not altered.

\begin{figure}[thpb]
  \centering	
  \includegraphics[width=\columnwidth]{Images/Rescaling2.pdf}
  \caption{Original $\theta(t)$ and rescaled position profiles $\theta(x)$, $\phi(x)$ with their corresponding torque equations.}
  \label{fig:rescaling}
\end{figure}

For what concerns the constraints, the rest-to-rest motion required zero speed $\dot{\phi}$ and acceleration $\ddot{\phi}$ in the start and endpoint:

\begin{equation} 
\begin{array}{ccccc}
\phi(-1)=-1 & , & \dot{\phi}(-1)=0 & , & \ddot{\phi}(-1)=0,\\
\phi(1)=1 & , & \dot{\phi}(1)=0 & , & \ddot{\phi}(1)=0.
\end{array}{}
\label{eq:constraints}
\end{equation}


Referring to \eqref{eq:position_function_cheb}, and by incorporating the motion profile constraints \eqref{eq:constraints}, the lower degree coefficients $[p_0,... , p_5]^T$ can be written as a function of the remaining coefficients $[p_6,... , p_n]^T$, such that $n-5$ degrees of freedom (DOF) are kept available for the optimization algorithm \cite{Hsu2014}. Thus, the energy optimal motion profile problem is formulated as the following minimization problem with design variable vector $\mathbf{o}=[p_6,... , p_n]^T$:

\begin{equation}
\begin{aligned}
& \underset{\mathbf{o} \, \in \, \mathbb{R}^{n-5}}{\text{minimize}}
& & T_{m;rms}(x) = \sqrt{\frac{1}{2}\int_{-1}^{1} {T_m(\phi(x,\mathbf{o}))}^2 \, \mathrm{d}x} .
\end{aligned}
\end{equation}

%Note that for some combinations of $\mathbf{o}$, the position profile $\theta(x)$ might be outside of the system property limits $0$ or $2\pi$. As these properties are only defined on the interval $[0,2\pi]$, this leads to unrealistic torque and objective values. To overcome this issue, a modulo operation on the motion profile $\theta(x)$ is used to map the angles to the system property interval.

In some applications, an additional constraint of zero jerk in the begin and endpoint can be imposed to limit the vibrations:

\begin{equation} \label{eq:constraint_jerk}
    \dddot{\phi}(-1)=0 \quad;\quad \dddot{\phi}(1)=0.
\end{equation}

Because of these two extra equations, the DOF is reduced to $n-7$ and the design variable vector can be expressed as $\mathbf{o}=[p_8,... , p_n]^T$.

\subsection{Initialization \& Design Space}
In this paper, the resulting optimization problem is solved with both a fast \textit{gradient-based} solver, the BFGS (Broyden–Fletcher–Goldfarb–Shanno) quasi-Newton method \cite{Nocedal2006}, and a global \textit{heuristic} solver, the genetic algorithm \cite{Holland1992}.

For gradient-based optimization, a starting point needs to be defined. The use of the Chebyshev basis $T_i(x)$ in representation \eqref{eq:position_function_cheb} allows initializing the optimization parameter vector at zero, since the coefficients in a convergent Chebyshev series development of the motion profile function $\theta(x)$ would converge to zero \cite{Majidian2017}. Here, we can safely assume some similar behavior for the coefficients $p_i$ in \eqref{eq:position_function_cheb}.

For what concerns the genetic algorithm, a similar approach is used for the initialization of the population. However, because a GA often samples a wide part of the design space \cite{Wenzhong2005}, it is beneficial to determine the exact bounds on the design vector $\mathbf{o}$. By doing so, the solver can cover a large part of the design space and reveal the global optimal solution. In the following paragraphs, thanks to the rescaled Chebyshev motion profile, strict bounds on the design vector $\mathbf{o}$ can be derived.

To define these bounds, we first introduce the integral $I$:

\begin{equation}\label{int}
	I = \int\limits_{0}^{2\pi} T_k(\cos\theta) \cos(\ell\theta) \, \mathrm{d}\theta.
\end{equation}

With respect to Eq. \eqref{eq:def_cheb_tri} and by using the inverse Simpson rule, the integral can be written as:

\begin{equation}
\begin{aligned}
	I &= \int\limits_{0}^{2\pi} \cos(k\theta) \cos(\ell\theta) \, \mathrm{d}\theta \\
	&= \frac{1}{2} \int\limits_{0}^{2\pi} \cos\big((k+\ell)\theta\big)\,\mathrm{d}\theta
	+ \frac{1}{2} \int\limits_{0}^{2\pi} \cos\big((k-\ell)\theta\big)\,\mathrm{d}\theta.
\end{aligned}
\end{equation}

The problem is divided into three cases of which the results will be used in the following paragraphs:
\begin{enumerate}

    \item \underline{$k+\ell = 0$} \\
    Since $k$ and $\ell$ are both positive, this is only possible for $k=\ell=0$. In this case, we find
    
    \begin{equation}\label{eq:case1}
        I = %\int\limits_{0}^{2\pi} \,\mathrm{d}\theta = 
        2\pi.
    \end{equation}
    
    \item \underline{$k-\ell = 0$} \\
    In this case, we find that $k = \ell$, which means that
    
    \begin{equation}\label{eq:case2}
    \begin{aligned}
        I %&= \dfrac{1}{2} \int\limits_{0}^{2\pi} \cos\big((k+\ell)\theta\big)\,\mathrm{d}\theta + \dfrac{1}{2} \int\limits_{0}^{2\pi} \,\mathrm{d}\theta \\
	%&= \dfrac{1}{2} \left[ \dfrac{\sin\big( (k+\ell)\theta \big)}{k+\ell} \right]_0^{2\pi} + \pi 
	= \pi.
	\end{aligned}
    \end{equation}
    
    \item \underline{$k+\ell \neq 0$ and $k-\ell \neq 0$} \\
    In this case, $k \neq \ell$ and both are not 0 at the same time. For the integral we then find
    
    \begin{equation}\label{eq:case3}
    \begin{aligned}
        I %&= \dfrac{1}{2} \int\limits_{0}^{2\pi} \cos\big((k+\ell)\theta\big)\,\mathrm{d}\theta + \dfrac{1}{2} \int\limits_{0}^{2\pi} \cos\big((k-\ell)\theta\big)\,\mathrm{d}\theta \\ &= \dfrac{1}{2} \left[ \dfrac{\sin\big( (k+\ell)\theta \big)}{k+\ell} \right]_0^{2\pi} + \dfrac{1}{2} \left[ \dfrac{\sin\big( (k-\ell)\theta \big)}{k-\ell} \right]_0^{2\pi} 
        = 0.
    \end{aligned}
    \end{equation}
    
\end{enumerate}
 
Further, a second integral $F$ is introduced which is used later on to obtain the strict bounds. 

\begin{equation}  \label{eq:integralF}
    \begin{aligned}
    F &= \int\limits_{0}^{2\pi} \phi(\cos\theta)\cos(\ell\theta)\,\mathrm{d}\theta.
    \end{aligned}
\end{equation}

By taking into account \eqref{eq:position_function_cheb}, we find the following result:

\begin{equation} 
    \begin{aligned}
    F &= \int\limits_{0}^{2\pi} \left(\sum\limits_{k=0}^n p_k T_k(\cos\theta)\right)\cos(\ell\theta)\,\mathrm{d}\theta \\
	&= \sum\limits_{k=0}^n p_k \int\limits_{0}^{2\pi} T_k(\cos\theta) \cos(\ell\theta) \, \mathrm{d}\theta.
    \end{aligned}
\end{equation}

Then, by taking into account \eqref{eq:case3}, only the term for which $k=l$ remains in the summation:

\begin{equation}
    \begin{aligned}
    F = p_\ell \int\limits_{0}^{2\pi} T_\ell(\cos\theta) \cos(\ell\theta) \, \mathrm{d}\theta.
    \end{aligned}
\end{equation}

This can be split into two cases. For $\ell = 0$ and with respect to \eqref{eq:case1} and \eqref{eq:integralF} we find:
\begin{equation}\label{c0}
	p_0 = \dfrac{1}{2\pi} \int\limits_{0}^{2\pi} \phi(\cos\theta)\,\mathrm{d}\theta,
\end{equation}

and for $\ell > 0$ with respect to \eqref{eq:case2} and \eqref{eq:integralF}:

\begin{equation}\label{cl}
	p_\ell = \dfrac{1}{\pi} \int\limits_{0}^{2\pi} \phi(\cos\theta)\cos(\ell\theta)\,\mathrm{d}\theta.
\end{equation}

For $\theta \in [0,2\pi]$, $\cos\theta$ lies in interval $[-1,1]$, so the image of $\phi(\cos\theta)$ also lies in the interval $[-1,1]$. Thus, we find:

\begin{equation}
	|p_0| \leq \dfrac{1}{2\pi}\int\limits_{0}^{2\pi} |\phi(\cos\theta)|\,\mathrm{d}\theta \leq \dfrac{1}{2\pi}\int\limits_{0}^{2\pi} \,\mathrm{d}\theta = 1.
\end{equation}

and

\begin{equation}
|p_\ell| \leq \dfrac{1}{\pi}\int\limits_{0}^{2\pi} |\phi(\cos\theta)||\cos(\ell\theta)|\,\mathrm{d}\theta \leq \dfrac{1}{\pi}\int\limits_{0}^{2\pi}|\cos(\ell\theta)| \,\mathrm{d}\theta.
\end{equation}

To calculate this last integral, we use the periodicity of the function $\cos(\ell\theta)$. This function has a period of $2\pi / \ell$, so goes $\ell$ times up and down on the interval $[0,2\pi]$. So, after taking the absolute value of this function, we find $2\ell$ times the integral over the positive part of a period, for example, the interval $[-\pi/2\ell, \pi/2\ell]$:

\begin{equation}
\begin{aligned}
    \dfrac{1}{\pi}\int\limits_{0}^{2\pi}|\cos(\ell\theta)| \,\mathrm{d}\theta = \dfrac{2\ell}{\pi} \int\limits_{-\pi/2\ell}^{\pi/2\ell} \cos(\ell\theta)\,\mathrm{d}\theta = \dfrac{4}{\pi}.
\end{aligned}
\end{equation}

Thus, the following bounds were obtained:

\begin{equation} \label{boundsDS}
    |p_0| \leq 1 \hspace{0.5cm} \text{ and } \hspace{0.5cm} |p_\ell| \leq \dfrac{4}{\pi}, \hspace{0.3cm} \ell =1,\dots,n.
\end{equation}

These constraints on the design space are exploited in the subsequent optimization.


